Fixed-Parameter Algorithms for Graph Constraint Logic

Non-deterministic constraint logic (NCL) is a simple model of computation based on orientations of a constraint graph with edge weights and vertex demands. NCL captures \PSPACE\xspace and has been a useful tool for proving algorithmic hardness of many puzzles, games, and reconfiguration problems. In particular, its usefulness stems from the fact that it remains \PSPACE-complete even under severe restrictions of the weights (e.g., only edge-weights one and two are needed) and the structure of the constraint graph (e.g., planar \textsc{and/or}\xspace graphs of bounded bandwidth). While such restrictions on the structure of constraint graphs do not seem to limit the expressiveness of NCL, the building blocks of the constraint graphs cannot be limited without losing expressiveness: We consider as parameters the number of weight-one edges and the number of weight-two edges of a constraint graph, as well as the number of \textsc{and}\xspace or \textsc{or}\xspace vertices of an \textsc{and/or}\xspace constraint graph. We show that NCL is fixed-parameter tractable (FPT) for any of these parameters. In particular, for NCL parameterized by the number of weight-one edges or the number of \textsc{and}\xspace vertices, we obtain a linear kernel. It follows that, in a sense, NCL as introduced by Hearn and Demaine is defined in the most economical way for the purpose of capturing \PSPACE.

==> ncl_poly.tex <==
\section{NCL with a single weight}
\label{sec:singleweight}

We show that \ncl with weights one and two as introduced by Hearn and
Demaine is minimal in the following sense: for any single weight $k \in
\Z_{\geq 1}$ the problem \nclk can be decided in polynomial time, hence at
least two weights are necessary to capture \PSPACE\xspace (assuming $\P \neq
\PSPACE$). For this purpose, we use a simple reduction to the problem of
finding a transformation between two common independent sets of two partition
matroids. We refer to this problem as \cis \reconfig and give a formal
definition shortly. We give a polynomial-time algorithm for this problem by
reducing it to the problem \textsc{$b$-Matching Reconfiguration}, which is
known to admit a polynomial-time algorithm~\cite{M:15}. In fact, a reduction to
the problem \textsc{Matching Reconfiguration} can be obtained by using the
construction given in~\cite{Shiloach:81}. Note that a polynomial-time algorithm
for \cis \reconfig implies polynomial-time algorithms for a range of other
interesting problems, see for instance~\cite[Chapter 41.2]{Schrijver:03}.


We recall some definitions related to partition matroids in order to define the
problem \cis \reconfig.  A partition matroid on a (finite) ground-set
\groundset is given by a partition $(S_i)_{i \in I}$ of $X$ and a tuple $d \in
\mathbb{Z}_{\geq 0}^I$, where $I$ is an index set. A subset $F \subseteq X$ is
called \emph{independent} if for $i \in I$, we have $|F \cap S_i| \leq d_i$.
That is, in any independent subset of \groundset, we may pick at most $d_i$
items from part $S_i$.  Let  $M_1, M_2$ be two partition matroids given by $M_1
= (\groundset, \mathcal{S}_1, d^1)$ and $M_2 = (\groundset, \mathcal{S}_2,
d^2)$, where $\mathcal{S}_1 = (S_i)_{i \in I}$ and $\mathcal{S}_2 = (S_j)_{j
\in J}$ are two partitions of a ground-set \groundset, $d^1 \in \nat_0^{I}$,
and $d^2 \in \nat_0^{J}$. We say that $F \in X$ is a \emph{common independent
set} of $M_1$ and $M_2$ if it is independent in $M_1$ and $M_2$. Let $S, T
\subseteq X$ be two common independent sets of $M-1$ and $M_2$. We say that $S$
and $T$ are \emph{adjacent} if their symmetric difference contains exactly one
item. Furthermore, a sequence $A_0, A_1, \ldots, A_\ell$ of common independent
sets of $M_1$ and $M_2$ is called \emph{reconfiguration sequence from $S$ to
$T$} if $A_0 = S$, $A_\ell = T$ and for $1 \leq i < \ell$, $A_i$ is adjacent to
$A_{i+1}$. The problem \cis \reconfig is defined as follows:
\begin{quote}
	\cis \reconfig\\
	\textbf{input:} Two partition matroids $M_1 = (\groundset,
	\mathcal{S}_1, d^1)$ and $M_2 = (\groundset, \mathcal{S}_2, d^2)$
	over a ground-set $X$, common
	independent sets $S, F \subseteq X$, and number $k \in \nat$.\\
	\textbf{question:} Is there a reconfiguration sequence from $S$ to $T$ such that each set in the sequence has cardinality at least $k-1$?
\end{quote}

Given an instance of \cis \reconfig, we construct a bipartite multigraph
$G_{M_1, M_2}$, such that the common independent sets of $M_1$ and $M_2$
corresponds to the $b$-matchings of $G_{M_1, M_2}$.  Let $M_1$ (resp. $M_2$)
be given by $M_1 = (\groundset, (S_i)_{i \in I}, d^1)$ (resp., $M_2 =
(\groundset, \mathcal{S}_2 = (S_j)_{j \in J}, d^2)$, such that the two index
sets $I$ and $J$ are disjoint. The vertex set of $G_{M_1, M_2}$ is $I + J$ and
for $i \in I$ and $j \in J$, the set $E(i, j)$ of edges joining $i$ and $j$ in
$G_{M_1, M_2}$ is given by $E(i, j) := S_i \cap S_j$. To obtain an instance of
the $b$-matching problem, we add capacities $b \in \nat^{I+J}$ to the vertices
of $G_{M_1, M_2}$ as follows:
For $i \in I$, let $b_i = d^1_i$ and for $j \in J$, let $b_i = d^2_i$
otherwise. It is readily seen that a common independent set $S$ of $M_1$ and
$M_2$ corresponds to a $b$-matching of $G_{M_1, M_2}$ and vice versa. 
\todo[inline]{TODO: explanation in the next paragraph}
Let us consider a reconfiguration graph $\matchgraph(G_{M_1, M_2})$ of
$b$-matchings of cardinality at least $k-1$ in $G_{M_1, M_2}$. That is, the
vertex set of $\matchgraph(G_{M_1, M_2})$ is the set of $b$-matchings of
cardinality at least $k-1$ in $G_{M_1, M_2}$. 
We
observe that, by construction, the
We note
that for the purpose of reconfiguration we have not gained or
lost anything by the transformation given above, since it is readily verified that the graphs
$\cisgraph(M_1, M_2)$ and $\matchgraph(G_{M_1, M_2}, b)$ are canonically
isomorphic.

\begin{proposition}
    \label{prop:bmatching:iso}
  %The graphs $\cisgraph(M_1, M_2)$ and $\matchgraph(G_{M_1, M_2}, b)$ are isomorphic.
    Two vertices $S$ and $T$ are adjacent in $\cisgraph(M_1, M_2)$ if and only if they are adjacent in $\matchgraph(G_{M_1, M_2})$.
  %The identity map on $\groundset$ induces an isomorphism of the graphs
    %The graphs $\cisgraph(M_1, M_2)$ and $\matchgraph(G_{M_1, M_2}, b)$ are isomorphic.
  %Any common independent set of $M_1$ and $M_2$ is a $b$-matching in $\mathcal{G}_{M_1,M_2}$, and
  %vice versa. Furthermore, for any $k \geq 1$, $S$ and $T$ are adjacent in $\cisgraph$ if and only if 
  %the symmetric difference of two $b$-matchings has
  %size at most two if and only if the corresponding common independent sets of
  %$M$ and $N$ are adjacent in $\mathcal{G}_{M,N}$.
\end{proposition}

A polynomial-time algorithm for \cis \reconfig now follows from the
polynomial-time algorithm for $ab$-constrained subgraph reconfiguration given
in \cite{M:15}. 
\begin{theorem}
	\cis \reconfig admits a polynomial-time algorithm.
	\label{thm:cis:polytime}
\end{theorem}
\todo[inline]{Proof.}

We now give the main result of this section.

\begin{theorem}
    For $k \in \Z_{\geq 1}$, \nclk admits a polynomial-time algorithm.
  \label{thm:nclk:ptime}
\end{theorem}
\begin{proof}
  Let $I = (G, d, w, \alpha, \beta)$ be an instance of \nclk.
  Observe that for $v \in V$, that the in-weight at $v$ is at least $d_v$ if
  and only if the out-weight of $v$ is at most the total weight of the arcs
  incident to $v$ minus $d_v$. By rearranging and dividing by $k$ it follows
  that the in-weight at $v$ is at least $d_v$ if and only if $\outdeg(v) \leq
  \outdeg(v) + \indeg(v) - \lceil d_v/k \rceil$. Now we can follow the
  construction given in~\cite[Chapter 41.2]{Schrijver:03} and define two
  partition matroids $M_1$ and $M_2$ on the ground-set $\groundset$, where
  \[
    \groundset := \bigcup_{\{v,w\} \in E} \{vw, wv\} \enspace.
  \]
  The independent sets of $M_1$ and $M_2$ are given by
  \begin{align*}
    \I(M_1) :=& \{ F \subseteq \groundset \mid |F\ \cap \{vw, wv\}| \leq 1, \{v, w\} \in E\} \\
    \I(M_2) :=& \{ F \subseteq \groundset \mid |F \cap \outarcs(v)| \leq \indeg(v) + \outdeg(v) - \lceil d_v/k \rceil\} 
  \end{align*}
  Observe that $\alpha$ and $\beta$ are common independent sets of $M_1$ and
  $M_2$ of cardinality $|E(G)|$. Consider common independent sets of $M_1$ and
  $M_2$ of cardinality at least $|E(G)|-1$. Suppose that any two such sets are
  adjacent iff their symmetric difference contains precisely one item. Then,
  due to the structure or $\I(M_1)$, any distance-two neighbors in the
  corresponding reconfiguration graph differ precisely with respect to the
  orientation of a single arc. We invoke Theorem~\ref{thm:cis:polytime} to
  solve the instance $(M_1, M_2, \alpha, \beta, |E|-1)$ of \cis \reconfig in
  polynomial time.
\end{proof}

\todo[inline]{Clean up the proof.}







